A RAG-Based Multi-Agent LLM System for Natural Hazard Resilience and Adaptation

Large language models (LLMs) are a transformational capability at the frontier of artificial intelligence and machine learning that can support decision-makers in addressing pressing societal challenges such as extreme natural hazard events. As generalized models, LLMs often struggle to provide context-specific information, particularly in areas requiring specialized knowledge. In this work we propose a retrieval-augmented generation (RAG)-based multi-agent LLM system to support analysis and decision-making in the context of natural hazards and extreme weather events. As a proof of concept, we present WildfireGPT, a specialized system focused on wildfire hazards. The architecture employs a user-centered, multi-agent design to deliver tailored risk insights across diverse stakeholder groups. By integrating natural hazard and extreme weather projection data, observational datasets, and scientific literature through an RAG framework, the system ensures both the accuracy and contextual relevance of the information it provides. Evaluation across ten expert-led case studies demonstrates that WildfireGPT significantly outperforms existing LLM-based solutions for decision support.

==> Beaverton_mitigation_policy_interaction.tex <==
assistant: Hello! Thank you for coming to discuss wildfire risk
management and the impact of climate change. Before we proceed further,
I'll need to ask you a few questions. This helps us tailor our
consultation to your specific needs and concerns. If you're unsure about
any question, feel free to say ``I don't know.'' Let's start with the
first question:

May I know what your professional background is?

user: I am an urban planner

assistant: Thank you for sharing that. Next question:

What are your primary concerns or questions about wildfires?

user: I am interested in how to manage development to mitigate
fire-related hazard risk. I am an urban planner in Beaverton, Oregon,
just outside Portland.

assistant: That's a crucial area to focus on, especially given your
role. Now, can you specify the exact location of concern for assessing
wildfire risks in terms of Latitude and Longitude? If you don't have
this information, I can help locate Beaverton, Oregon, on the map.

user: Sure show me the map

assistant: Please confirm the location by clicking the `Confirm
Location' button on the map provided for Beaverton, Oregon. Let me know
once you've confirmed it.

user: The location has been confirmed: latitude 45.48366474908892,
longitude -122.80603408813478.

assistant: Thank you for confirming the location. Next, could you
specify the urgency or timeline for addressing your concerns about
wildfire risks?

user: This is for a long-term community plan. The timeline is 30 years.

assistant: Understood, a long-term perspective is essential for
sustainable urban planning regarding wildfire management. Lastly, are
there specific aspects of wildfire risks that you are particularly
interested in exploring?

user: Can you provide some examples?

assistant: Certainly! Some specific aspects you might consider include:

\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\tightlist
\item
  \textbf{Fire Behavior Modeling:} Understanding how wildfires spread
  based on terrain, vegetation, and climate conditions.
\item
  \textbf{Building Codes:} Reviewing or developing building regulations
  to enhance fire resistance in urban design.
\item
  \textbf{Evacuation Routes:} Planning effective evacuation procedures
  and routes to enhance public safety.
\item
  \textbf{Infrastructure Resilience:} Enhancing resilience of public
  utilities and services against fire damage.
\item
  \textbf{Community Education:} Programs to educate residents about fire
  prevention and safety.
\end{enumerate}

Which of these areas, or any others, do you find most pertinent to your
work as an urban planner?

user: I'm interested in Building Codes and Infrastructure Resilience

assistant: Thank you for specifying your interests. Let me summarize the
information gathered:

\begin{itemize}
\tightlist
\item
  \textbf{Profession:} Urban planner
\item
  \textbf{Concern:} Interested in managing development to mitigate
  fire-related hazard risks
\item
  \textbf{Location:} Beaverton, Oregon (Latitude: 45.48366474908892,
  Longitude: -122.80603408812478)
\item
  \textbf{Time:} 30-year timeline for a long-term community plan
\item
  \textbf{Scope:} Focused on Building Codes and Infrastructure
  Resilience
\end{itemize}

I will share this checklist with you now to confirm all details are
correct. Here it is:

\begin{itemize}
\tightlist
\item
  \textbf{Profession:} Urban planner
\item
  \textbf{Concern:} Interested in managing development to mitigate
  fire-related hazard risks
\item
  \textbf{Location:} Beaverton, Oregon (Latitude: 45.48366474908892,
  Longitude: -122.80603408812478)
\item
  \textbf{Time:} 30-year timeline for a long-term community plan
\item
  \textbf{Scope:} Building Codes and Infrastructure Resilience
\end{itemize}

Please let me know if all details are accurate or if there's anything
else you'd like to adjust.

user: Yes this is accurate

assistant: Based on our previous discussions and the specific concerns
you have as an urban planner focusing on building codes and
infrastructure resilience in Beaverton, Oregon, here is the customized
plan to help assess and mitigate wildfire risks for your long-term
community plan:

\subsubsection{Step 1: Data Analysis}\label{step-1-data-analysis}

\begin{itemize}
\tightlist
\item
  \textbf{Dataset:} Long Term Fire History Records

  \begin{itemize}
  \tightlist
  \item
    I will analyze this dataset to identify patterns or cycles in
    wildfire activity over the years in and around Beaverton.
    Understanding historical trends is crucial for anticipating future
    wildfire scenarios and their potential impact on urban areas.
  \end{itemize}
\end{itemize}

\subsubsection{Step 2: Literature
Search}\label{step-2-literature-search}

\begin{itemize}
\tightlist
\item
  \textbf{Scope:} Research on building codes and infrastructure
  resilience in wildfire-prone areas

  \begin{itemize}
  \tightlist
  \item
    I will conduct a literature review to gather insights from
    scientific studies and case studies relating to effective methods
    for constructing fire-resilient buildings and infrastructure. This
    includes architectural innovations, materials, and design strategies
    proven to mitigate fire risk.
  \end{itemize}
\end{itemize}

\subsubsection{Step 3: Recommendations}\label{step-3-recommendations}

\begin{itemize}
\tightlist
\item
  \textbf{Deliverables:} A comprehensive report including analysis
  results, literature review findings, and practical recommendations

  \begin{itemize}
  \tightlist
  \item
    Based on the analysis of the historical fire data and the findings
    from current research, I will compile actionable recommendations
    tailored to enhance Beaverton's resilience against wildfires. This
    includes proposed updates to building codes and suggestions for
    infrastructure improvements.
  \end{itemize}
\end{itemize}

This plan is designed to arm you with a data-driven foundation and
research-backed strategies that align with Beaverton's development goals
while ensuring long-term safety and sustainability in the face of
wildfire risks.

Do you have any questions or concerns about this plan? Would you like to
discuss any specific elements in more detail or add anything else to the
approach?

user: As for the dataset, could you analyze fire weather index instead?

assistant: Absolutely, analyzing the Fire Weather Index (FWI) can indeed
provide valuable insights, particularly in anticipating future fire risk
conditions, which is essential for your focus on building codes and
infrastructure resilience. Here's how we could incorporate the FWi into
our plan:

\subsubsection{Step 1: Data Analysis}\label{step-1-data-analysis-1}

\begin{itemize}
\tightlist
\item
  \textbf{Dataset:} Fire Weather Index (FWI)

  \begin{itemize}
  \tightlist
  \item
    I will analyze the FWI focusing on both current trends and
    projections for the mid-century (2045-2054) to assess the potential
    increase in fire danger due to climate change. This will help
    predict more dangerous periods or seasons for wildfires around
    Beaverton.
  \end{itemize}
\end{itemize}

\subsubsection{Step 2: Literature
Search}\label{step-2-literature-search-1}

\begin{itemize}
\tightlist
\item
  I will continue to search for literature on effective building codes
  and infrastructural designs that enhance resilience to wildfires,
  ensuring that they align with the predictions derived from the FWI
  analysis.
\end{itemize}

\subsubsection{Step 3: Recommendations}\label{step-3-recommendations-1}

\begin{itemize}
\tightlist
\item
  Based on the trends identified in the FWI and insights from the
  literature, I will provide tailored recommendations. These will focus
  on updating building codes, infrastructure planning, and possibly
  adjusting urban development strategies to mitigate the heightened fire
  risks identified for future decades.
\end{itemize}

Does this adjustment to the plan meet your expectations? Would you like
to discuss any specific elements in more detail, or is there anything
else you'd like to add to the approach?

user: Looks good

assistant: The Fire Weather Index (FWI) projections for Beaverton,
Oregon, indicate a generally stable fire risk from historical periods
into the mid-century, with minor fluctuations across the seasons.
Specifically, the historical FWI (1995 - 2004) shows:

\begin{itemize}
\tightlist
\item
  Spring: Low risk (FWI = 2.0)
\item
  Summer: Medium risk (FWI = 14.92)
\item
  Autumn: Medium risk (FWI = 12.3)
\item
  Winter: Low risk (FWI = 0.59)
\end{itemize}

Looking into the mid-century (2045 - 2054), the projected values are:

\begin{itemize}
\tightlist
\item
  Spring: Low risk (FWI = 1.94)
\item
  Summer: Medium risk (FWI = 14.15)
\item
  Autumn: Medium risk (FWI = 12.81)
\item
  Winter: Low risk (FWI = 0.56)
\end{itemize}

Although there's a slight decline in summer and an increase in autumn
risks, the area remains mostly in the low to medium fire danger
category. These predictions are essential for planning as they imply
that fire-related hazards might not drastically increase, but continuous
monitoring and mitigation approaches should still be prioritized to
address these consistent fire risks.

You can view more detailed data and methodology at the Climate Risk \&
Resilience Portal: \url{https://disgeoportal.egs.anl.gov/ClimRR/}.

Would you like to delve deeper into any specific season or aspect of
these projections, or shall we proceed with the next steps, such as
reviewing relevant literature for urban planning strategies against fire
hazards?

user: Let's review some relevant literature

assistant: In addressing the pressing issue of wildfire resilience in
urban areas, researchers and urban planners have proposed various
strategies that resonate closely with concerns for communities like
Beaverton, Oregon.

\textbf{Constanza Gonzalez-Mathiesen and Alan March (2018)} emphasize
that urban planning can significantly enhance wildfire resilience by
adopting design principles focused on physical resistance and
facilitating response (Gonzalez-Mathiesen \& March, 2018). Such
principles can be integral to developing more robust building codes and
ensuring that urban infrastructure in Beaverton is attuned to withstand
fire threats.

\textbf{Crystal Kolden and Carol Henson (2019)} provide a compelling
case study from Montecito, California, during the 2017 Thomas Fire,
showcasing the efficacy of community-wide mitigation strategies. They
highlight that robust community partnerships and proactive mitigation
efforts substantially reduced vulnerability and damage despite extreme
conditions (Kolden \& Henson, 2019). This example sets a benchmark for
Beaverton's approach towards community involvement and pre-fire
preparations.

\textbf{Stephen R. Miller et al.~(2016)} discuss both regulatory and
non-regulatory tools that communities can employ to manage wildfire
risks effectively. Covering a range of options from zoning codes to
educational platforms, this guide provides a comprehensive resource for
municipalities to customize their strategies based on specific local
needs (Miller et al., 2016).

Each paper underscores the multifaceted approach needed to tackle
wildfire risks effectively, blending regulation, community action, and
informed urban planning to safeguard urban interfaces.

\subsubsection{References:}\label{references}

Gonzalez-Mathiesen, C., \& March, A. (2018). Establishing Design
Principles for Wildfire Resilient Urban Planning. DOI:
\href{https://doi.org/10.1080/02697459.2018.1429787}{10.1080/02697459.2018.1429787}

Kolden, C., \& Henson, C. (2019). A Socio-Ecological Approach to
Mitigating Wildfire Vulnerability in the Wildland Urban Interface: A
Case Study from the 2017 Thomas Fire. DOI:
\href{https://doi.org/10.3390/fire2010009}{10.3390/fire2010009}

Miller, S. R., et al.~(2016). Planning for Wildfire in the
Wildland-Urban Interface: A Resource Guide for Idaho Communities. DOI:
\href{https://doi.org/10.2139/ssrn.2845046}{10.2139/ssrn.2845046}

Would you like further analysis or specific case studies from these
papers to refine our strategy for Beaverton's urban planning?

user: Yes, could you please provide additional information on regulatory
or policy tools that communities can use to manage wildfire risks?

assistant: In the discourse of wildfire management, recent literature
emphasizes a variety of regulatory and policy tools that communities can
adopt to safeguard against wildfire risks effectively.

\textbf{Paulo M. Fernandes et al.~(2020)} critique the lack of dynamic
approaches within wildfire regulation policies. They suggest that
evolving from fire exclusion to integrated fire management practices is
essential. Their analysis indicates that recognizing wildfires as
complex socio-ecological processes rather than mere natural hazards can
significantly influence policy effectiveness (Fernandes et al., 2020).
This perspective opens the door for Beaverton to reimagine its wildfire
policies, ensuring that they are adaptive and holistic.

\textbf{John Heineke and Stein Weissenberger (1974)} explore
decision-making models to minimize wildfire risks in urban areas. They
propose tailor-made policy decisions based on specific data sets that
could help manage wildland activities efficiently, preventing ignitions
and reducing potential losses (Heineke \& Weissenberger, 1974). This
method could be particularly beneficial for Beaverton in formulating
data-driven policies that adapt to local wildfire dynamics.

\textbf{Stephen R. Miller et al.~(2016)} further enrich this dialogue by
discussing specific regulatory and non-regulatory tools available to
manage wildfire risks. They highlight the importance of comprehensive
urban planning mechanisms like zoning codes, building codes, and
community wildfire protection plans. Additionally, they suggest
leveraging educational platforms like Firewise to enhance community
awareness and preparedness (Miller et al., 2016). This comprehensive
approach could serve as a blueprint for Beaverton, integrating
educational outreach with stringent regulatory measures to foster a
safer urban environment.

\subsubsection{References:}\label{references-1}

Fernandes, P. M., et al.~(2020). Wildfire policies contribution to
foster extreme wildfires. DOI:
\href{https://doi.org/10.1016/b978-0-12-815721-3.00010-2}{10.1016/b978-0-12-815721-3.00010-2}

Heineke, J., \& Weissenberger, S. (1974). An Analysis of Wildfire
Prevention. DOI:
\href{https://doi.org/10.1109/tsmc.1974.4309359}{10.1109/tsmc.1974.4309359}

Miller, S. R., et al.~(2016). Planning for Wildfire in the
Wildland-Urban Interface: A Resource Guide for Idaho Communities. DOI:
\href{https://doi.org/10.2139/ssrn.2845046}{10.2139/ssrn.2845046}

Would you like a deeper exploration into any specific regulatory models
or further guidance on implementing these tools in Beaverton's urban
planning?

user: What are some specific changes to zoning codes and/or building
codes that communities can make to manage wildfire risk?

assistant: To effectively manage wildfire risks in communities like
Beaverton, Oregon, specific changes to zoning codes and building codes
can be integral. Here are some recommended strategies tailored to
enhance resilience against wildfires:

\subsubsection{Zoning Codes
Adjustments:}\label{zoning-codes-adjustments}

\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\tightlist
\item
  \textbf{Defensible Space Zones}: Create zoning regulations that
  mandate defensible spaces around properties, classified into different
  zones with specific vegetation management requirements to reduce fire
  fuel.
\item
  \textbf{Buffer Zones}: Implement zoning that incorporates buffer zones
  between wildland areas and urban developments. These areas can be
  managed to have low fire fuel vegetation or be used for agricultural
  purposes that naturally resist fire spread.
\item
  \textbf{Land Use Planning}: Restrict or carefully control development
  in high-risk wildfire areas. This might include limiting the types of
  allowable constructions or the density of buildings to reduce
  potential fire damage.
\end{enumerate}

\subsubsection{Building Codes
Enhancements:}\label{building-codes-enhancements}

\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\tightlist
\item
  \textbf{Fire-Resistant Materials}: Mandate the use of fire-resistant
  materials for roofing, siding, and other exterior parts of buildings.
  Products rated as Class A, such as certain types of metal, tiles, or
  specially treated wood, offer the highest resistance against fire.
\item
  \textbf{Egress and Access}: Revise building codes to ensure that there
  are multiple egress routes for residents and adequate access routes
  for emergency services. This is crucial for both safety during
  evacuations and effective firefighting operations.
\item
  \textbf{Landscaping Regulations}: Enforce guidelines on landscaping in
  residential and commercial properties to include fire-resistant plants
  and to maintain safe distances between vegetation and buildings.
\end{enumerate}

\subsubsection{Combination of Regulatory and Design
Approaches:}\label{combination-of-regulatory-and-design-approaches}

\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\tightlist
\item
  \textbf{Cluster Development}: Allow for cluster housing developments
  that concentrate buildings in safer areas, reducing the interface with
  high-risk fire zones and thus minimizing the overall community's
  vulnerability.
\item
  \textbf{Incentives for Retrofitting}: Provide incentives, such as tax
  reductions or grants, for property owners to retrofit existing
  structures with fire-resistant designs and materials.
\item
  \textbf{Emergency Infrastructure}: Integrate requirements for
  fire-adapted infrastructure, including water supply systems designed
  for firefighting, like static water tanks and increased hydrant
  availability.
\end{enumerate}

\subsubsection{Community Engagement and
Enforcement:}\label{community-engagement-and-enforcement}

\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\tightlist
\item
  \textbf{Regular Inspections and Compliance}: Implement regular
  inspections to ensure compliance with new codes and provide
  educational resources to property owners about the importance and
  benefits of adherence. 2 \& policies**: Ensure that all zoning and
  building policy changes are developed in consultation with fire
  departments, urban planners, and community members to create
  sustainable and widely supported frameworks.
\end{enumerate}

Implementing these changes requires careful consideration of local
conditions and should be supported by comprehensive planning and
community engagement. These adjustments are designed not only to
mitigate the impact of potential wildfires but also to foster a
resilient urban environment where the community feels prepared and
protected.

Would you like assistance with developing specific policy drafts or
planning community engagement strategies to introduce these changes?

user: Are there supporting literature for Buffer Zones?

assistant: The utility of buffer zones in wildfire management is
increasingly recognized in urban planning for its effectiveness in
mitigating fire risks. Recent scholarly work points to vital insights
that can guide communities like Beaverton in integrating these zones
within their developmental strategies.

\textbf{Greg Penney and Steven Richardson (2019)} explore innovative
models that address the underestimate of radiant heat flux in urban
areas with small vegetation fires. Their research underscores the
significance of properly designed urban spaces that act as buffer zones,
reducing the impact of wildfires in densely populated localities (Penney
\& Richardson, 2019). This approach demonstrates the potential of buffer
zones to enhance resilience by mitigating fire spread and intensity
before it reaches critical urban assets.

\textbf{Maureen Kennedy and Morris Johnson (2014)} investigate the
effects of fuel treatments as buffer zones during Arizona's 2011 Wallow
Fire. Their analysis shows that these zones significantly lowered fire
severity and provided firefighters better management options, thereby
protecting urban interfaces (Kennedy \& Johnson, 2014). This evidence
supports the adjustment of spatial planning to include strategic buffer
zones that reduce wildfire transmission to urban areas.

\textbf{A. Gill and Scott Stephens (2009)} discuss the challenges and
multifaceted benefits of integrating asset protection zones, which act
similarly to buffer zones, in urban-wildland interfaces. They highlight
planning strategies that combine urban development with natural
landscape management to minimize fire risk impacts efficiently (Gill \&
Stephens, 2009). This work suggests that Beaverton would benefit from a
holistic approach that balances fire protection, biodiversity, and
residential needs.

\subsubsection{References:}\label{references-2}

Penney, G., \& Richardson, S. (2019). Modelling of the Radiant Heat Flux
and Rate of Spread of Wildfire within the Urban Environment. DOI:
\href{https://doi.org/10.3390/fire2010004}{10.3390/fire2010004}

Kennedy, M., \& Johnson, M. (2014). Fuel treatment prescriptions alter
spatial patterns of fire severity around the wildland--urban interface
during the Wallow Fire, Arizona, USA. DOI:
\href{https://doi.org/10.1016/j.foreco.2014.01.014}{10.1016/j.foreco.2014.01.014}

Gill, A., \& Stephens, S. (2009). Scientific and social challenges for
the management of fire-prone wildland -- urban interfaces. DOI:
\href{https://doi.org/10.1088/1748-9326/4/3/034014}{10.1088/1748-9326/4/3/034014}

Would you like to explore more about implementing these strategies in
Beaverton's urban planning framework?


==> conclusions.tex <==
%In conclusion, we have developed an LLM agent, WildfireGPT, representing a step forward in leveraging language models for specialized scientific domains such as climate change, with a particular focus on wildfire risks. This prototype shows great potential in transforming user queries into actionable insights, offering a customized interactive experience through strategic questioning and planning, and accessing climate projection data alongside scientific literature in climate science.  {\it Domain expert feedback underscores WildfireGPT's strengths in defining the scope of inquiries, establishing a clear roadmap for discussions, and enhancing productivity through efficient data retrieval and interpretation, which would be very time-consuming for a user to accomplish independently. }%Overall, the LLM agent was effective in providing user-specific information by pulling from literature and actual climate projections, which would be very time-consuming for a user to accomplish independently. 
%Furthermore, we identify several key areas for  future work, such as redundant questioning, gaps in user profiling, the need for more relevant data, and the refinement of recommendation strategies.

